Automated Transpilation of Imperative to Functional Code using Neural-Guided Program Synthesis (Extended Version)

While many mainstream languages such as Java, Python, and C# increasingly incorporate functional APIs to simplify programming and improve parallelization/performance, there are no effective techniques that can be used to automatically translate existing imperative code to functional variants using these APIs. Motivated by this problem, this paper presents a transpilation approach based on inductive program synthesis for modernizing existing code. Our method is based on the observation that the overwhelming majority of source/target programs in this setting satisfy an assumption that we call trace-compatibility: not only do the programs share syntactically identical low-level expressions, but these expressions also take the same values in corresponding execution traces. Our method leverages this observation to design a new neural-guided synthesis algorithm that (1) uses a novel neural architecture called cognate grammar network (CGN) and (2) leverages a form of concolic execution to prune partial programs based on intermediate values that arise during a computation. We have implemented our approach in a tool called NGST2 and use it to translate imperative Java and Python code to functional variants that use the Stream and functools APIs respectively. Our experiments show that NGST2 significantly outperforms several baselines and that our proposed neural architecture and pruning techniques are vital for achieving good results.

==> pruning.tex <==
\section{Trace Compatible Pruning}
\label{sec:prune}

The goal of pruning is to decide if a partial program candidate $C$ is consistent with an input program trace $\tau(P, \sigma)$ of input program $P$ on initial input valuation $\sigma$. \footnote{For the rest of the section, we use $\tau$ as shorthand for $\tau(P, \sigma)$.} Our pruning technique is inspired by \cite{polikarpova2016program} and more generally bidirectional type checking \cite{pierce2000local}, which combines top-down and bottom-up propagation of type constraints. In our context, we adapt this style of rules to propagate output constraints down the tree, and trace constraints up the tree.

Similar to bidirectional type checking, we introduce two judgements: an \textit{output} judgement $\ojudge{\tau, \sigma}{e}{v}$ which states that expression $e$ generates value $v$ given trace $\tau$ and valuation $\sigma$, and a \textit{trace} judgement $\tjudge{\tau, \sigma}{e}{V}$ which states that expression $e$ generates some value $v \in V$ given trace $\tau$ and valuation $\sigma$. Intuitively, we can think of output judgements as stating that expression $e$ \textit{must} have some output value $v$, and trace judgments as stating that expression $e$ \text{may} have one of the output values $v \in V$ as suggested by trace $\tau$.

Similar to round-trip type checking from \cite{polikarpova2016program}, we depart from bidirectional type checking in how we apply top-down versus bottom-up constraint propagation. In bidirectional type checking, constraints are propagated top-down exhaustively, and then bottom-up. In our system, we interchange top-down and bottom-up propagation freely. In this vane, we introduce a new \textit{consistency} judgement $\conjudge{\tau, \sigma}{e}{v}$ which states that an expression $e$ generates a value $v$ which is consistent with the bottom-up constraint that $v \in V$ (as shown in rule $\updownarrow$ in Figure~\ref{fig:conrule}).

\begin{figure}
    \centering
    $\irule{
      \tjudge{\tau, \sigma}{e}{V} \;\;\; \ojudge{\tau, \sigma}{e }{v} \;\;\; v \in V
    }{\conjudge{\tau, \sigma}{e}{v}}$  [$\updownarrow$-RULE] 
    \caption{Consistency Judgement Rule}
    \label{fig:conrule}
\end{figure}

\subsection{Output Rules}

\begin{figure}
    \centering
    \begin{tabular}{c}
    \textbf{Output Rules $\downarrow$} \\~\\
    $\irule{
      \conjudge{\tau, \sigma}{e_1}{[x_1, ..., x_n]} \;\;\; \conjudge{\tau, \sigma[i \mapsto x_j]}{e_2}{y_j}
    }{\ojudge{\tau, \sigma}{map(e_1, \lambda i. e_2)}{[y_1, ..., y_n]}}$  [MAP-$\downarrow$] \\~\\
    $\irule{
      \bfrac{
        \conjudge{\tau, \sigma}{e_1}{[x_1, ..., x_k]} \;\;\; 
        subsequence([y_1, ..., y_n],[x_1, ..., x_k])
      }{
        \bfrac{
          if \; (x_j \notin y) \; then \; (\conjudge{\tau, \sigma[i \mapsto x_j]}{e_2}{false}) \;\;\;
        }{
          if \; (x_j \in y) \; then \; (\conjudge{\tau, \sigma[i \mapsto x_j]}{e_2}{true})
        }
        }
    }{\ojudge{\tau, \sigma}{filter(e_1, \lambda i. e_2)}{[y_1, ..., y_n]}}$  [FILTER-$\downarrow$] \\~\\
    $\irule{

    }{\ojudge{\tau, \sigma}{N}{v}}$  [NONTERM-$\downarrow$] \\~\\    
    $\irule{
      \llbracket f(i_1, ..., i_n)[\sigma]] \rrbracket = v
    }{\ojudge{\tau, \sigma}{f(i_1, ..., i_n)}{v}}$  [FUNC-$\downarrow$] \\~\\    
    \end{tabular}
    \caption{Bidirectional Output Rules}
    \label{fig:checkrules}
\end{figure}

Figure~\ref{fig:checkrules} gives the rules for propagating output constraints down programs in our DSL. For example, the MAP-$\downarrow$ rule states that an expression $map(e_1, \lambda i.e_2)$ can produce a list $[y_1, ..., y_n]$ if $e_1$ is consistent with some list $[x_1, ..., x_n]$, and for each $x_j \in [x_1, ..., x_n]$, $e_2$ is consistent with value $y_j$ when it's argument $i$ is mapped to $x_j$. Informally, this rule states that each element of the output of map should correspond to the result of applying $e_2$ to an element of $e_1$.

The rule FILTER-$\downarrow$ states that an expression $filter(e_1, \lambda i. e_2)$ can produce a list $[y_1, ..., y_n]$ if $e_1$ is consistent with some list $[x_1, ..., x_n]$, $[y_1, ..., y_n]$ is a subsequence of $[x_1, ..., x_n]$, and each $y_j$ corresponds to values of $[x_1, ..., x_n]$ on which $e_2$ is consistent with $true$. Informally, this rule states that each element of the output of filter should correspond to an element of $e_1$ for which $e_2$ returned $true$.

The rules FLATMAP-$\downarrow$, FIND-$\downarrow$, and FOLD-$\downarrow$ are of a similar flavor, and can be found in the appendix. The rule NONTERM-$\downarrow$ states that a non-terminal is unconstrained, that is, it can produce any value. The rule FUNC-$\downarrow$ states that a function application produces the value it creates when executed (according to semantics $\llbracket . \rrbracket$).

\subsection{Trace Rules}

\begin{figure}
    \centering
    \begin{tabular}{c}
    \textbf{Trace Rules $\uparrow$} \\~\\
    $\irule{
      \bfrac{
        \tjudge{\tau, \sigma}{e_1}{V_{e_1}} \;\;\;
        \forall \; [x^l_1, ..., x^l_k] \in V_{e_1}. \; \tjudge{\tau, \sigma[i \mapsto x^l_j]}{e_2}{V^l_{j}}    
      }{
        V^l = \{[v^l_1, ..., v^l_k] \; | \; v^l_j \in V^l_j\} \;\;\;
        V = \bigcup {V^l}
      }

    }{\tjudge{\tau, \sigma}{map(e_1, \lambda i. e_2)}{V}}$  [MAP-$\uparrow$] \\~\\
    $\irule{
      \bfrac{
        \tjudge{\tau, \sigma}{e_1}{V_{e_1}} \;\;\;
        \forall \; [x^l_1, ..., x^l_k] \in V_{e_1}. \; \tjudge{\tau, \sigma[i \mapsto x^l_j]}{e_2}{V^l_{j}}    
      }{
        V^l = \{[x^l_m, ..., x^l_w] \; | \; true \in V^l_j\} \;\;\;
        V = \bigcup {V^l}
      }
    }{\tjudge{\tau, \sigma}{filter(e_1, \lambda i. e_2)}{V}}$  [FILTER-$\uparrow$] \\~\\
    $\irule{
    V = \{ \llbracket f(i_1, ..., i_n)[\sigma] \rrbracket \; | \; \sigma' \in \tau \land \sigma = \sigma'\}
    }{\tjudge{\tau, \sigma}{f(i_1, ..., i_n)}{V}}$  [FUNC-$\uparrow$] \\~\\
    $\irule{
    shared(N) \;\;\;
    \exists t. \; V = \{ \llbracket t[\sigma] \rrbracket \; | \; \sigma' \in \tau \land \sigma = \sigma'\}
    }{\tjudge{\tau, \sigma}{N}{V}}$  [SHARED-NONTERM-$\uparrow$] \\~\\
    % $\irule{
    % \bfrac{
    %   \neg shared(N) \;\;\;
    % }{
    %   \bfrac{
    %     \tjudge{\tau, \sigma}{map(e_1, \lambda i. e_2)}{V_{map}} 
    %   }
    %   {
    %     \bfrac{
    %       \tjudge{\tau, \sigma}{filter(e_1, \lambda i. e_2)}{V_{filter}}
    %     }{
    %       \bfrac{
    %         ...
    %       }{
    %         V = V_{map} \cup V_{filter} \cup ... \cup V_{fold}
    %       }
    %     }
    %   }
    % }
    % }{\tjudge{\tau, \sigma}{N}{V}}$  [NONSHARED-NONTERM-$\uparrow$] \\~\\
    $\irule{
      \neg shared(N) \;\;\;
    }{\tjudge{\tau, \sigma}{N}{\mathcal{U}}}$  [NONSHARED-NONTERM-$\uparrow$] \\~\\  
    \end{tabular}
    \caption{Bidirectional Trace Rules}
    \label{fig:tracerules}
\end{figure}

Figure~\ref{fig:tracerules} gives the rules for propagating trace constraints up programs in our DSL, which mirror the output rules from Figure~\ref{fig:checkrules}.

Informally, rule MAP-$\uparrow$ states that map can produce any value which results from applying some value of $e_2$ to elements of a possible value of $e_1$. Note, we use the notation $\{[v^l_1, ..., v^l_k] \; | \; v^l_j \in V^l_j\}$ to indicate the set of all possible lists of length $k$ constructed by taking possible values of $e_2$ applied to elements of $e_1$.

The rule for filter, FILTER-$\uparrow$, is very similar to MAP-$\uparrow$. The only difference is that the values which map can produce are not the result of what $e_2$ produces, but rather the values of $e_1$ on which $e_2$ could produce $true$. The reader should note that the notation here simplifies a bit, because unlike map where we produce possible lists of length $k$, here we must consider all lists of length $\leq k$.

The trace rules FLATMAP-$\uparrow$, FILTER-$\uparrow$, FIND-$\uparrow$, and FOLD-$\uparrow$ are of a similar flavor, and can be found in the appendix.

Rules FUNC-$\uparrow$ and SHARED-NONTERM-$\uparrow$ are where the trace is actually used. The rule FUNC-$\uparrow$ states that the possible values a function application $f(i_1, ..., i_n)$ can take on is limited to the values it took on in the input trace $\tau$ in the same context $\sigma$. This rule is sound as a consequence of the trace compatibility assumption. The rule SHARED-NONTERM-$\uparrow$ is similar, stating that a shared nonterminal can only take on values of some term $t$ in the input trace in the same context $\sigma$.

The final rule, NONSHARED-NONTERM-$\uparrow$ states that a non-shared nonterminal is unconstrained. That is, a non-shared nonterminal can take on any value from the universal set $\mathcal{U}$.

\subsection{Pruning Algorithm}

Our pruning algorithm falls naturally out of the bidirectional derivation rules given in Figures~\ref{fig:checkrules} and \ref{fig:tracerules}. Figure~\ref{fig:prunealg} shows the pruning algorithm.

\begin{figure}
\begin{algorithm}[H]
    \begin{algorithmic}[1]
        \Procedure{Prune}{}
            \State \textbf{input:} Source program $\mathcal{P}$
            \State \textbf{input:} Candidate program $\mathcal{C}$
            \State \textbf{input:} Test inputs $\mathcal{I}$
            \vspace{0.05in}
            \For{$x \in \mathcal{I}$}
                \State $\tau := \tau(\mathcal{P}, x)$
                \State $v := \llbracket P \rrbracket_x$
                \If{$\nojudge{\tau, x}{\mathcal{C}}{v}$}
                    \State \Return $\bot$
                \EndIf
            \EndFor
            \vspace{0.05in}
            \State \Return $\top$
    \EndProcedure
    \end{algorithmic}

\end{algorithm}
\vspace{-0.3in}
\caption{Pruning Algorithm}  
\label{fig:prunealg}
\end{figure}

As input, the pruning procedure takes the source program $\mathcal{P}$, the candidate partial program to check $\mathcal{C}$,
and a set of test inputs $\mathcal{I}$ use to generate traces. The algorithm iterates through each input $x \in \mathcal{I}$, and uses that input to determine $\tau$, the trace of the input program, and $v$, the desired output. It then uses the bidirectional rules above to check if $\mathcal{C}$ can produce the desired output $v$, given the input $x$ and source program trace $\tau$, i.e., $\ojudge{\tau, x}{\mathcal{C}}{v}$. If the candidate cannot produce the desired output, it is pruned (i.e. returns $\bot$). Otherwise, if the candidate can possibly satisfy all test inputs $\mathcal{I}$, the algorithm returns true ($\top$).

\begin{theorem} [Pruning Soundness]
If \textsc{Prune}$(\mathcal{P}, \mathcal{C}, \mathcal{I})$ returns $\bot$, $\mathcal{C}$ is inconsistent with $\mathcal{P}$; that is, there exists no completion of $\mathcal{C}$ s.t. $\mathcal{C}$ is equivalent to $\mathcal{P}$.
\end{theorem}

==> scratch.tex <==
\begin{figure}[t]
  \centering
  \begin{tabular}{c}
           Concolic Semantics $\symexec{\cdot}$ \\
           \\ 
  $\begin{array}{lll}
  \symexec{\mathrm{map}}([\symexp_1, \ldots, \symexp_k], \{\symexp_1 \rightarrow \symexp_1^\prime, \ldots, \symexp_k \rightarrow \symexp_k^\prime\}) & \defeq & y = [\symexpsub_1^\prime, \ldots, \symexpsub_k^\prime] \\
  \symexec{\mathrm{filter}}([\symexp_1, \ldots, \symexp_k], \{\symexp_1 \rightarrow \symexp_1^\prime, \ldots, \symexp_k \rightarrow \symexp_k^\prime\}) & \defeq & (\neg \symexpsub_1^\prime \land \neg \symexpsub_2^\prime \land \ldots \land \neg \symexpsub_k^\prime) \rightarrow (y = []) \\
  & & \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \land \ldots \land \\
  & & (\symexpsub_1^\prime \land \symexpsub_2^\prime \land \ldots \land \symexpsub_k^\prime) \rightarrow (y = [\symexpsub_1, \ldots, \symexpsub_k]) \\
  \symexec{\mathrm{flatmap}}([\symexp_1, \ldots, \symexp_k], \{\symexp_1 \rightarrow [\symexp_{11}^\prime, \ldots, \symexp_{1l_1}^\prime], \ldots, \\
  \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \symexp_k \rightarrow [\symexp_{k1}^\prime, \ldots, \symexp_{kl_k}^\prime]\}) & \defeq & y = [\symexpsub_{11}^\prime, \ldots, \symexpsub_{1l_1}^\prime, \ldots, \symexpsub_{k1}^\prime, \ldots, \symexpsub_{kl_k}^\prime] \\
  \symexec{\mathrm{find}}([\symexp_1, \ldots, \symexp_k], \symexp_0, \{\symexp_1 \rightarrow \symexp_1^\prime, \ldots, \symexp_k \rightarrow \symexp_k^\prime\}) & \defeq & (\symexpsub_1^\prime \rightarrow \symexp_1) \land \ldots \land (\symexpsub_k^\prime \rightarrow \symexp_k) \land \\
  & & (\neg \symexpsub_1^\prime \land \ldots \land \neg \symexpsub_k^\prime \rightarrow \symexp_0) \\
  \symexec{\mathrm{fold}}([\symexp_1, \ldots, \symexp_k], \symexp_0, \{(\symexp_0, \symexp_1) \rightarrow \symexp_1^\prime, \\
  \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ (\symexp_1^\prime, \symexp_2) \rightarrow \symexp_2^\prime, \ldots \\
  \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ (\symexp_{k-1}^\prime, \symexp_k) \rightarrow \symexp_k^\prime\}) & \defeq & ((k=0) \rightarrow \symexp_0) \land ((k > 0) \rightarrow \symexp_k^\prime)
  \end{array}$ \\
  \\
  Inverse Concolic Semantics $\symexecback{\cdot}{-i}$ \\
  \\
  \todo{add inverse semantics} \\
  \\
  Notation \\
  \\
  $\begin{array}{lll}
  y = [\symexp_1, \ldots, \symexp_k] & \equiv & \exists x_1, \ldots, x_k. \ y = [x_1, \ldots, x_k] \land \symexp_1[x_1/y] \land \ldots \land \symexp_k[x_k/y] \\
  \symexpsub & \equiv & \symexp[y^\prime/y] \ \ \ \text{where} \ \ \mathrm{FreshVar}(y^\prime)
  \end{array}$
  
  \end{tabular}
 \vspace{-0.1in}
  \caption{Concolic semantics $\symexec{\cdot}$ and inverse concolic semantics $\symexecback{\cdot}{-i}$ for \fdsl \todo{give weaker forward semantics for filter? Like some sort of inclusion?}}
  \label{fig:concolicSemantics}
  \vspace{-0.15in}
\end{figure}

